Learning by Teaching: Key Challenges and Design Implications

Benefits of learning by teaching (LbT) have been highlighted by previous studies from a pedagogical lens, as well as through computer-supported systems. However, the challenges that university students face in technology-mediated LbT$\unicode{x2013}$whether it be teaching oneself, teaching a peer, or teaching an agent$\unicode{x2013}$are not well understood. Furthermore, there is a gap in knowledge on the challenges that students encounter throughout the process of teaching (content selection, preparation, teaching, receiving and giving feedback, and reflection) despite its importance to the design of LbT platforms. Thus, we conducted a study with 24 university students where they taught content they had not fully grasped, without guidance, and participated in a semi-structured interview. Results demonstrate that participants encountered the following challenges: psychological barriers relating to self and others, and lack of know-how. Furthermore, we illuminate design implications required to overcome these challenges and benefit from LbT without requiring prior training in pedagogy.

==> 7-tools.tex <==
% \section{Students' Feature Recommendations \& Opinions for Web-Based LbT Platform Tooling}
% could be shortened
% todo: summary of the recommendations and categorize them and a count of the feature preferences (e.g. ppl rec these 5-6 things and here's what they said about each and how many wanted it) 

% in paper include summary of the recommendations and categorize them and a count of the feature preferences (e.g. ppl rec these 5-6 things and here's what they said about each and how many wanted it) 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Scaffolding and System Support %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% focusing on tools that will help with overcoming the struggles
% \subsection{Technology Support for Teaching Unfamiliar Material}

%removed Jan12: We are interested in discovering features that would be necessary or desirable for supporting LbT activities (e.g. content preparation, finding peers, teaching, receiving and giving feedback, etc.). During the interview, we attempted to gauge whether participants would be comfortable with the features and if they could see themselves actually using them. We also asked participants whether they would adopt specific features (e.g., lesson templates, peer matching) for a LbT platform if it exists. Towards the end of this chapter, we also present an early stage prototype that incorporates design solutions outlined in Chapter 5 to begin exploring LbT platform designs for university students. 
% removed for Aug 22 : One of the main goals of our study is need-finding: we are interested in discovering features that would be necessary or desirable for supporting learning-by-teaching activities (e.g. content preparation, finding peers, teaching, receiving and giving feedback, etc.). During the interview, we attempted to gauge whether participants would be comfortable using the features and if they could see themselves actually using them. We also asked participants whether they would adopt specific features (e.g., lesson templates, tutor-tutee matching) for a learning-by-teaching platform if it exists.

% what is this feature/platform exactly? What would it look like? How would it be used? - what information on this were participants given?

% removed Jan12:
% \begin{figure*} [h]
%   \centering
%   \includegraphics[width=.8\columnwidth]{Figure web-based tools supporting lbt.png}
% %   \caption{Preferred Configuration Types for Learning-by-Teaching Sessions}
% \caption{Students' perceived benefits and concerns when using web-based tools supporting LbT}
%   \label{toolssummary}
% \end{figure*}


% \subsection{Tools for Teaching Preparation}  

% Figure \ref{toolssummary} displays a summary of participants opinions on various features. The first section of this chart, breaks down their views on using tools for teaching preparation. Most participants said that they would be comfortable using a web based support tool to help prepare for their LbT session through a guide or template aimed to help students generate content or lesson plans (P2-8, P10-25). The table also provides a list of participant's perceived benefits of such tools (e.g. content organization). P4 also mentioned such tools would make the process of preparing ``easier'' for ``someone who hasn't done it before''. In addition to the concerns listed in the table, other participants' preference to use preparation tools depends on a few considerations. P6 would use preparation tools if they ``knew the material'' and were going to teach someone who did not (i.e. regular teaching), but would not use them to teach material that the they themselves do not understand. This is a recurring theme, with P10, P13, and P22 expressing similar opinions that they would not use them if the purpose was to learn the material for themselves through teaching, instead of ensuring the audience learns something.
% While many participants commented on the benefits of using preparation tools, the design should avoid solutions that might discourage their use (e.g. lacking flexibility) and carefully consider the balance between the amount of effort and time needed to use these tools.

%  in thesis:
% Most participants said that they would be comfortable using a web based support tool to help prepare for their LbT session through a guide or template aimed to help students generate content or lesson plans (P2-8, P10-25). Such tools could help them with document preparation for planning the structure (P3), organization (P8, P20, P24), or timing (P12), lesson material standardization (P4, P17) and expectations (P11, P17), getting better at making content (P5) or notes (P19), making their own notes more ``consolidated and cohesive" (P7), breaking down content (P18), and with template ideation (P24) design by teaching experts (P14). P4 also mentioned such tools would make the process of preparing ``easier'' for ``someone who hasn't done it before''.
% On the contrary, a few participants gave reasons for not wanting to use such tools, including perceiving it as an ``overhead'' (P2) and wanting ``to have freedom'' instead of being ``restrained'' (P21). P15 perceived such tools as not useful for their own learning (as a teacher) since they ``like learning at [their] own pace''.
% For other participants, their preference to use preparation tools depends on a few considerations. P6 would use preparation tools if they ``knew the material'' and was going to teach someone who did not, but would not use them just to teach material that the teachers themselves do not understand. This variability in the purpose of the teaching activity is a recurring theme, with P10, P13 and P22 expressing similar opinions that they would not use if the purpose was to learn the material themselves through teaching, instead of ensuring the audience learns something.
% In summary, while many participants commented on the benefits from using preparation tools if they were available, the design of such tools should avoid features that might discourage their use (e.g., by lacking flexibility), and carefully consider the balance between the amount of effort and time needed to use these tools, and the additional learning progress they provide to both teachers and listeners. 

% ##################################### Extra notes ########################
% 2.1
% removed for Aug 22 : \subsection{Support for Teaching Preparation}  

% removed for Aug 22 : Most participants said that they would be comfortable using a web based support tool to help prepare for their learning-by-teaching session through a guide or template aimed to help students generate content or lesson plans (P2-8, PP10-25) and one participant said they might be comfortable using it (P9). Out of these participants, those who would actually use it (P3-5, P7-8, P11-14, P17-20, P24) it would help them with document preparation for planning the structure (P3), organization (P8, P20, P24), or timing (P12), lesson material standardization (P4, P17) and expectations (P11, P17), getting better at making content (P5) or notes (P19), making their own notes more ``consolidated and cohesive" (P7), breaking down content (P18), and with template ideation (P24) design by teaching experts (P14).

% removed to cut down pages:In terms of support that they might expect in such a guidance tool, P12 said they can imagine a tool that prompts you to think about ``what background information might you need", or ``what words might you have to make sure [that they] are understood by both parties", or how to lay things out, from ``background information", to ``premise", to ``specifics of the problem", to ``steps to solve" and ``abstracting from" the problem. P8 also said they would want to know the ``background knowledge that you would need for this topic", ``the main points" of the topic, and the ``evidence for the main points", presented in the ``hamburger model". Another participant, P12 said the template prompts ``might depend a bit on the topic but I could imagine they're being ... what background information might you need to like verify with the person" listening to the session, and ``what words might" you want to ``make sure are understood by both parties", ``specifics of the problem and then from there like the steps to solve, and maybe from abstraction from that if there's like almost like theorems to take away that were used specifically in the question". A third participant, P18, also mentioned wanting a prompt for ``prerequisite information". P14 also wanted to include ``like boxes of information" for the ``title", ``lesson objectives, so like the summary of ... what we're teaching, and then like a clear like step one, step two, step three, ..." process.

% p8 yy (no ``the only case i can see is if it's like a really disjointed and confusing template then i might not use it") include background and hamburger info ``what do you expect to see in this kind of template P: i definitely would want to see like what's the background knowledge that you need for this topic and what are the main points that you have for the topic uh what are the pieces of evidence for your main points it's almost like i don't know if you heard like the hamburger model that they used to teach in elementary school R: yeah P: similar to that where they kind of just organize your paragraph or your topic and they say what are you going to discuss what are your points for that where does the evidence come from"
% P12 for time planning, including background, list specifics of problem, step by step sol, then abstract take aways `` yeah i think that'd be helpful to actually because i'm sure the the concept would probably be a set amount of time and so having a template would help you probably set up for that so i would be comfortable with that and i would use it (R: okay) i like templates 
% p14 yes depending on the depth of inform, beneficial if the templates are made by ppl who know more about teaching than them and have a better understanding of how to present information. might include course title, lesson objectives, step by step teaching, gradually getting harder and to more advanced content
% p18 breaking down `` title of the lesson the prerequisite information that would be taught before the lesson the breakdown I'm not sure how it would prompt you to put in the breakdown maybe if it gave you an option to not compartmentalize but like separate separate your lesson plan into different parts I'm not sure what else it would prompt that probably be it from what I can imagine ``

% removed for Aug 22 : A few participants mentioned that such a template for a learning-by-teaching platform would be able to provide standardization to the teaching methods and set expectations. For example, P11 said the guide/template for teaching helps to set the `expectation', but the types of prompts would depend on the subject being taught. Furthermore, P17 said ``If this ... content preparation component helps standardize the expectations, then I think it's more beneficial to both teachers and the students". 
% removed to cut down pages:"I feel like this is a good way for people to understand the question ....but when, if you think about like an online platform like uh without some kind of standardization people bring in like all kinds of different formats, so make it a standard, or like uh or improve user experience I think overall". 
% removed for Aug 22 : Lastly, P4 said, ``I think building a standardized method for sharing content and teaching is easy for someone who's actually having to build that teaching content" but for ``someone who hasn't done it before it's really hard to start from nowhere but having some sort of like template makes it easier". P4 even said that ``it's very annoying when everyone's changing the way they put material together. Some of them don't write enough, some of them write a lot, some of them don't even share slides, like that it's just really confusing so having a more standardized method helps."
% p4 standardization... annoying when profs have diff ways of making slide decks, drag drop content, everyone is changing the way they put together material. helps the student doing the learning by teaching ..."i think building a standardized method for sharing content and teaching is easy for someone who's actually having to build that teaching content someone who hasn't done it before it's really hard to start from nowhere but having some sort of like template makes it easier" 
% P17 improve ux ``if this of this content pro preparation component helps standardize the expectations then I think it's more beneficial to both teachers and the students" ... some more on
% P11 to set expectations of how to use new platform ** `` i think if i were going to use the platform i would definitely like to have some sort of template to yeah just to know an expectation R: what kind of prompts would you expect to see on such a template P: ....

% yy
% quotes below are only in first para briefly
% p3  prep documentation and structure of course um i guess like i ... if it's already in my workflow for example if i already say use my ipad a lot then it would be useful for example if i want to maybe draw something or you know sketch something out then a tablet would be very helpful in preparing my documentation for that ...  structure: that would be very helpful in that like i kind of i guess have an idea of when to what the structure of the the thing's going to be so that would be helpful yeah 
% P20 organization ``absolutely and then I think the organizational tool helps especially if it's not something that I'm say it's say for example it's a whole unit that somebody's struggling with or it's a whole unit that we have to cover for an exam having an organized lesson plan and a guide that"
% p24 `` yes I would use it because I love templates and I love like tools that allow you to organize anything that you're about to do so yes" and they would want to explore other templates to find things they didn't think about and then make the best one

% p5 to get better at making the content they would annotate the lesson plan and make it interactive ``to get better at it and i would i annotate take also to maybe some concept and okay i think it's good to have like a touch screen that you can like annotate and then to be very interactive uh using that lesson plan"

% P19 yes because it's smth their trying to work on `` I'm trying to be better at making notes and stuff so I think having that template would help a lot already"

% p7 use it for their own notes too ``yeah i feel like that would be really  good because it kind of gives you like an outline of how to format  the different things you want to talk  about makes it more like consolidated and cohesive  so i feel like that would be pretty good  and I'd probably use it not just for  learning by teaching but  if if that was like what people use for learning by teaching i would assume that  it's  useful in other applications so I'd  probably just use it for my own notes even if i wasn't teaching"


% ========

% comfortable
% y p2 p3 p4 p5 P6 p7 p8 p10 p11 p12 P13 p14 p15 p16 P17 P18 P19 p20 p21 p22 p23 p24 p25
% n
% p9

% removed for Aug 22 : On the contrary, some participants said they would be comfortable with this feature but would not use it (P2, P15, P21, P23). Participants expressed this because it ``seems like a lot of work, like overhead" (P2), ``because [they] don't like temp, like well ... [they] want to have freedom ... to create [their] own lesson plans .... having it there is nice, but [they] just don't like to be restrained/restricted by the lesson plan" (P21), or simply because ``it's not that useful for [them]" (P23). P15 said, ``I don't really think I would benefit from having some extra scaffolding and I'd rather just learn it the way I want to learn it" because ``generally I prefer like learning at my own pace".
% use
% y p3 p4 p5 p7 p8 P11 p12 p13 p14 P17 P18 P19 p20 p24
% n p2 p15 p21 p23
% maybe P6 p9 p10 p13 p16 p22 p25

% yn
% p2  yn it seems like a lot of work and a lot of overhead 
% p15 prob wouldn't benefit from it and wants to learn how they wanna do it
%  p21 ``because I don't like temp like well I like I want to have freedom like I want to create my own lesson plans having it having it there is nice but I just don't like to be restrained restricted by the lesson plan"
%  P23 ``it's not that useful I don't know it's not that useful for me"

% removed for Aug 22 : Lastly, the rest of the participants said they might use this feature (P6, P9-10, P13, P16, P22, P15). P10 said that his willingness to use such a feature would depend on what his goals are: ``if I'm trying to study myself, I probably wouldn't use it; but if I was using it for tutoring purpose, then I probably would... if I'm tutoring, I feel like there's a more of a responsibility for me to organize how things are gonna go, like what order I'm gonna be teaching things; whereas if I'm just studying on my own, I wouldn't find it necessary to go through all that work just to plan out what I'm going to be learning." Another participant, P6 said ``if I was actually if I knew the material and I was teaching it to somebody that didn't understand, then i would use the lesson plan" however ``if the point of this [platform] was so that you would teach material that you don't understand then i don't really get the point of having a lesson plan". Other participants said that their usage would depend on how ``stringent" the guide was (P9), if they were ``genuinely teaching and for catering to diff styles" (P13), if the ``viewer is trying to get something from it" (P16) and ``maybe they don't like [their] slides" (P16), or ``[depending] on ... how fast [they] need to learn the material and how much effort [they] want to put into it" (P25). Lastly P22 said, ``my goal in using this platform---I assume---would be to improve my knowledge by teaching, right, and if I'm not getting so much back then I want to you know maybe use different venues or different templates of teaching to see if I can identify those gaps better whereas if I am already you know identifying lots of gaps as I teach and brightening my knowledge then I don't think there's a need for me to you know change the way that I'm teaching."

% ym
% p6 ym would only use it for actual teaching not lbt ``um yeah i think like it'd be helpful to know but i also feel like if if the point of this was so that you would teach material that you don't understand then i don't really get the point of having a lesson plan R: okay and do you think this is something you might use  P: i think like if i was actually if i knew the material and i was teaching it to somebody that didn't understand then i would use the lesson plan"
% p9 ym ``probably but it depends on the the stringentness of the template because there's a really depending on the topic there's a really weird balance between having a really stringent guide and breaking down the material in a way that makes sense because it could be by time it could be by concept it could be by resources it could be like a timeline going through things like it depends if it's a thematic analysis or like they have different breakdowns i guess of what you're trying to teach `` .. more for the e.g.
% p10 [usage] would depend on what my goals are like if i'm trying to study myself that i probably wouldn't use it but if yeah like if i was using it for like a tutoring purpose then i probably would. if i'm tutoring i feel like there's a more of a responsibility for me to kind of organize how things are gonna go and like what order i'm gonna be teaching things whereas if i'm just studying on my own i wouldn't find it necessary to go through that all that work just to you know plan out what i'm going to be learning"
% p13 yym would like to have the option to use it, helpful for genuinely teaching and for catering to diff styles but that might not fit in certain templates, but you'd have to prep rather than study
% p16 use it for learning by teaching for themselves but not for teaching someone else ``whether I think I would use it and I'd say maybe is that if the purpose is for me to learn through teaching preparing slides on my own accord and putting the things down that I think are important and the structure that I think is interesting will make it more useful to me but then if it's in that the viewer is trying to get something from it maybe they don't learn the same way that I do and maybe they don't like my slides so yeah a maybe"
% P22 maybe if the feedback they get is stuff they already knew ... ``then I would go in and use it because I think you know my my goal in using this platform I assume would be to improve my my knowledge by teaching right and if I'm not getting so much back then I want to you know maybe use different venues or different templates of teaching to see if I can identify those gaps better whereas if I am already you know identifying lots of gaps as I teach and brightening my knowledge then I don't think there's a need for me to you know change the way that I'm teaching"
% P25  *"I'd be comfortable using it because it might like provide some structure to the lesson whether I'd actually use it I'm not I think depends on like how fast I need to learn the material and how much effort I want to put into it like if something I already know pretty well then I feel like I would just rather talk about it but if it's something that like my thoughts are kind of scattered then I would appreciate using it"

% not yet included - don't know what the template would include p13 p19





% =============================================================================
% previously Tools for LbT in Various Configurations (+2 subsections). moved to previous section 
% =============================================================================


% removed Jan12:
% \subsection{Tools for Teaching during the LbT Sessions}
% % 2.3-------------------------------------------------------------------------------------------
% In Figure \ref{toolssummary}, we outline various tools that can be used to support the teaching activities during students' LbT sessions. For each of these tools, the figure outlines their perceived benefits and concerns for using this tool. For screen sharing, all participants who were specifically asked about it (P2-4, P6-8, P10-14, P16-25) said that they would use it, however, one participant didn't use it for their LbT session. 
% removed for Aug 22 :  P18 noticed that ``it's like pretty constant at this point especially with COVID so I think everyone's comfortable and uses it at this point so I think it'd be good to carry that forward because it's a useful tool." 
% A few participants specifically pointed out that it would be beneficial for math sessions (P6-7, P19, P23) where there it is  ``very computational" and ``[has] a lot of notations" (P23) or when trying to code and show various programs (P12).
% removed for Aug 22 : saying that ``there are certain topics... that are just better if you can just show something... math are very like computational very have a lot of notations" (P23). 

% removed Jan12: P12 explained that they didn't use this tool during their session due to concerns of ``security risks" and the concern of users using this ``for academic dishonesty" when matched with their peers in the same courses.

% removed for Aug 22 :  However, P12 said ``I'd use it. The only thing is that can there's a few security risks about that. uh so that's just that's the only thing I can think about in terms of why that might be a bad thing to include in pieces of software uh especially with I could imagine people using that for like uh academic dishonesty. I could see that people trying to match with people in the same course and like sharing course notes but hopefully that wouldn't be a problem but that's like other than that I think that's a useful tool especially if you're trying to teach like coding or something where you can't quite teach it on a whiteboard you might want to actually show specific programs." 
% removed Jan12: Another participant also shared some concerns, P13 said ``there's technical issues like when you share they don't see it or vice versa, or you don't know what you're sharing like which screen or desktop, or it slows slows down your Wi-Fi. It would be more comfortable if you knew exactly what you were screen sharing and you could double check."
% 18 - q everyone
% 6 - qm
% 7 -qm
% 19 - q m
% 23 -q m
% 12 - q ad
% 13 - q13 diff
% \noindent {\bf Whiteboard and Concept Mapping Tools. }
% yy P2-4, P6-7, P10, P12-13, P15, P18-20, P23
% Of the 21 participants who were asked about whiteboard tool or concept map tools, many of them said that they would be comfortable with using it and would use it (P2-4, P6-7, P10, P12-13, P15, P18-20, P23).
% removed Jan12: For whiteboard and concept mapping tools, one participant (P23) said that they would like to ``be able to use [their] Apple Pencil" but a ``big problem is [that they] currently don't know how to screen share [their] iPad to [their] laptop, so [they] ...don't do it... There should be an easy way for people to [do so]."
% removed to cut down pages:P10 said that they could see himself using an annotation tool during both the preparation phase of teaching or in the live teaching session, explaining ``if I have a really complicated topic, I feel like it would be beneficial to have that laid out already. I could see myself doing that in the preparation phase; whereas if it's more important to the topic---that they see the process, being built ... one step at a time before adding to that diagram---then I would probably use it during the actual lesson". Another participant, P12, said that it would have improved their teaching; ``I would use that. Actually, that's kind of something I completely skipped over when I was discussing, so I didn't actually use any teaching tools clearly ... and I mostly relied on my preference for how to break apart a problem but obviously my teaching would have been significantly better were I to use visual aids because no one can keep track of all this information, just in their mind, but I don't have any. So but yeah, that's where a tool like that would come in useful, where I actually had the setup of being matched with someone to teach and there's built in visual aids that I can use and create images with to actually teach people." 
% removed for Aug 22 : Another participant (P18) said that for concept maps, ``if I'm trying to come up with an idea start from a base and then keep building off of it so mostly ideas and projects are probably where I'd use that, not just course material." P4 said that from the perspective of the student who is doing the learning-by-teaching, ``if [they] don't use it, it means they probably understood the topic already and [they] didn't have to actually draw, explain, and write."
% P18 concept maps `` if I'm trying to come up with an idea start from a base and then keep building off of it so mostly ideas and projects are probably where I'd use that, not just course material"
%P23 ``big problem is if I like currently I don't know how to screen share my iPad to my laptop so I basically don't do it I guess there should be like an easy way for people to"
% p4 examples annotate at the same time and ``if i don't use it it means they probably understood the topic already and i didn't have to actually draw explain and write"
% P12 would have made their teaching better ``yeah no i would use that actually that's kind of something i completely skipped over when i was discussing so i didn't actually use any teaching tools clearly and i mostly relied on my preference for how to break apart a problem but obviously my teaching would have been significantly better where i to use visual aids because no one can keep track of all this information just in their mind but i don't have any so but yeah that's where a tool like that would come in useful where i actually had the setup of being matched with someone to teach and there's built-in visual aids that i can use and create images with to actually teach people so yeah important tool"
% removed for Aug 22 : space removed
% removed Jan12: A few participants imagined this tool to be collaborative (P7, P15, P20). P20 described it as a ``way of illustrating ideas and it's ... very collaborative oriented---I mean---if you make it to be that way."
% Figure \ref{toolssummary} outlines other participants perceived benefits and concerns about these tools. In general, participants would like to be able to use this collaboratively, with specific peers, and features.
% P7 also suggested the idea of providing a lock where the student teaching could ``unlock it to give the others an opportunity to collaborate if they want to."  Similarly, P15 envisions that shared access with restrictions and added the concept of including ``an invisible maker, which only you ... can reveal later" which would be helpful when ``learning something about the graph theory, and ... there's many things you can do with drafts like you can connect them in different ways so say you want to connect them with some criterion".
% removed for Aug 22 : where ``everyone who's involved in that in that session should be able to access it, but maybe when one person is presenting only they can access it." They also thought of a specific use case where having ``an invisible maker, which only you ... can reveal later" would be helpful for ``learning something about the graph theory, and ... there's many things you can do with drafts like you can connect them in different ways so say you want to connect them with some criterion".
% P15 another thing which which could be helpful is you could sort of like I don't know maybe and this more applies to when you're teaching other people but you could sort of have like an invisible marker like which only you can see basically which which maybe you can reveal later which you don't necessarily feel like you could write the answer and hide it or if you're doing something where I mean I'm thinking of a very specific thing right now like a very specific application of this but like like do you want me to say that .... so if you were learning something about the graph theory and you want to like you want like there's many things you can do with drafts like you can connect them in different ways so say you want to connect them with some criterion like two like the edges are all different colors something like that like if you could kind of practice it just to make sure it's right or something like that I think that would be a helpful tool ... I think if you could because it's really hard to do these things in your head and especially if you if you want to come up with some examples just on the fly to say that it's not uncommon for this to happen like I can just think of an example in 10 seconds just to make sure I think that would be helpful and other than that maybe I know maybe you could like link textbooks or something like PDFs in general if you have the e-copy of some textbook you can link it to that so you can have the textbook show up side-by-side as you reference it ... so yeah I think maybe what what you could have instead of that is like have one public screen and one private screen so each person has their own like private screen where they can write whatever they want and so yeah I mean something like that so I don't think it's necessarily just the person who's teaching to have it"
% P20 ``un way of illustrating ideas and it's yeah it's very collaborative oriented I think I mean if you make it to be that way"
% 
% removed to cut down pages:A few participants said that they would be comfortable with this tool but they would not use it because of time (P8), how well it works (P8), and because of being able to screen share and pull up another software to work off of (P14). One participant, P8 said they would probably not use the whiteboard since on both computers and iPads ``it doesn't ever write as nicely and then it just feels like it takes up more time than is helpful", however, for ``the maps and things like that and dragging and dropping, I would totally use. I like having something that I can screen share and then I can have up for reference. It's just when it's writing, my writing will get too messy or it'll get all like jumbled together and I just don't I never liked that". One participant (P21) said that they would not be comfortable with this tool due to lack of access to drawing tablets but they would use it. 
% yn P8 ``um i don't think i'd probably use the whiteboard too much just because uh on computers and iPads it doesn't ever write as nicely and then it just feels like it takes up more time than is helpful but the maps and things like that and dragging and dropping i would totally use i like having something that i can screen share and then i can have up for reference it's just when it's writing my writing will get too messy or it'll get all like jumbled together and i just don't i never liked that in elementary school and high school so i don't do that anymore ``
% P14 `` no just because just because yeah if you have like screen sharing i think it's semi-irrelevant because they could pull up Microsoft Paint and work off of there" ... ``i think it's the same concept as screen sharing"
% ny P21 ``well like I have a laptop I don't have like an iPad pro or like a sketchable board so I'm actually not that comfortable because it's hard to use given my current technology restraint"
% removed for Aug 22 : 
% removed Jan12: While a few participants said that they would be comfortable with using it, they might use it depending on the situation (P9, P16-17, P25) or on the content they are teaching (P11).
% A few participants said that they would be comfortable with it but they might use it depending on the situation (P9, P16-17, P25) or on the content they are teaching (P11).
% For example, P25 said ``if I guess I had more time to prepare content" they would use it and
% removed for Aug 22 :  ``because I think it's more helpful to I guess like draw things out or explain like using diagrams and pictures." 
% P17 would use it on the condition that on their ``average attempts [they] have a good experience" and when ``something as well needs to be drawn" such as ``2d coordinates, that's not something [they] can type" so they would ``appreciate an existing  ... support for that; they don't want to go to like another software to like do the drawing". Similarly, P16, said ``I might just opt to screen share and use like Google Drawings instead or Paint but if it worked as well or better then yeah I'd use it if it was integrated." Lastly, P9 thought that ``[their] writing is very bad" and they would use it ``only if [they] had to like draw a figure".
% ym P9 ``my writing is very bad i would use it but only if i had to like draw a figure for some reason or draw something that wasn't text but I'd probably be knowing me mostly use text because I've tried to draw and it has thus far never worked out for me because i just can't do it like that's a me problem" P11 (depending on the course)
% P16 ``I might just opt to screen share and use like google drawings instead or paint but if it worked as well or better then yeah I'd use it if it was integrated"
% P17 ``uh yes I'm comfortable using it but I'm probably not going to use it unless like unless average attempts I have a good experience out of it and the really simple of being being I haven't really joined a whiteboard before if I'm explaining questions I also use words or write on piece of paper so something that I use on a regular basis `` .. ``something as well needs to be drawn a lot of times I have to draw something like when I was talking to you about like the 2d coordinates like that's not something I can type like you have to let people see the circle see the line if I just say there's a circle and there's a line you'd be like where is it right does it make much sense just to type it so yeah I i imagine some parts definitely needs to be drawn in order to explain the concepts `` ... if teaching prob need to use `` I appreciate an existing existing uh support for that I don't want to go to like another software to like do like the drawing and stuff"
% P25 
% \noindent {\bf Digital Screen Pointers.} 
% removed Jan12: For using digital screen pointers when teaching, several participants said they would feel comfortable with using this and would use it (19 of 21 participants) for the benefits listed in Figure \ref{toolssummary}. 
% of the 21 participants who were asked if they would be comfortable with using a digital screen pointer and if they would use it, many said yes (P2-5, P7, P9, P10, P12, P14-20, P22-25) so that they could draw attention to specific areas of a busy screen (P3), point out important parts of the diagrams (P10, P11) or to allow peers to give live feedback (P4, P10, P19) in combination with the screen sharing feature (P17, P22) or whiteboard feature (P23). P5 observed that on some video calling platforms, you cannot see the chat window in the same screen but they would like to and to be able to point to it. 
% removed for Aug 22 : P3 said it would be especially helpful if there's a `` whole lot of content on the screen" and they want to draw attention to a specific part.
% removed Jan12: One participant who outlined both benefits and concerns explained that during their LbT session, when using ``Photoshop, it's confusing if you don't have a mouse or a pointer because you can't just say 'this tool', 'that tool', 'oh go to the left side of your screen' because there's just so many calls to action ... and buttons all over the screen" but ``a regular mouse courser could get lost just because black on dark grey---I think Photoshop's dark grey---so if ... it was a bright red dot that would be helpful like a laser pointer almost" (P14).
% removed for Aug 22 : Similarly, P14 encountered that situation in their own learning-by-teaching session, they said when using ``Photoshop ...
% Similarly, P12 experienced difficulties when trying to indicate a specific location in a peer's code and there were no line numbers.
% removed for Aug 22 : P12 also had a similar experience and said ``I was actually helping someone with their code earlier today and I was trying to say 'oh over there, like that line', like because they didn't have line numbers on so they were like circling different lines with their mouse and I was just like I just want to point out my screen and tell you where it is so like I think that that would be very useful."
% yy P2-5, P7, P9, P10, P12, P14-20, P22-25
% 
% not included in detail P19 ``it'd be nice to have both the teacher and the or the person who's doing the learning by teaching to have it and also the learner having access to that um definitely different color pointers would be helpful or even a label actually not a label would be too much different colors or sizing"
% P12 ``when trying to have a conversation i was actually helping someone with their code earlier today and i was trying to say oh over there like that line like because they didn't have line numbers on so they were like circling different lines with their mouse and i was just like i just want to point out my screen and tell you where it is so like i think that that would be very useful for um on the like the other way around for someone for them both to be able to point at the work essentially um"
% P14
% P3 ``it would be helpful if there's maybe a whole lot of content on the screen that i need to maybe pinpoint or highlight or uh maybe like draw the attention to"
% P5 point to chat ``on zoom i believe you can see the cursor yeah it's just now from zoom you cannot see the you know the chat yeah uh when you see on the screen you cannot see the top banner part the other person cannot see it"
% P17 ``it works well when in combination with the screen sharing feature `` and P22 or whiteboard P23
% removed for Aug 22 : Lastly, two participants said that they would be comfortable with this tool but they may or may not use it depending on the situation (P8, P11). 
% removed for Aug 22 : P8 said it would depend on the design of the pointer; `` like a cursor or like circles that you can draw, I would totally use that. I just don't like their laser pointers in particular because you can't see them very well." The other participant P11 said that they would not ``if [they were] just trying to explain a theory or a concept. [They] don't think that [they] would need to, kind of indicate like this word pay attention to this word, like circle it or like aggressively underline" but they think that it would be useful ``if you're a biology student and you're trying to talk about different parts of a diagram or something".
% ym P8, P11
% P8 depending on the design: `` like a cursor or like circles that you can draw i would totally use that i just don't like their laser pointers in particular because you can't see them very well ``
% P11 ``if i was just um trying to explain a theory or a concept I don't think that i would need to kind of indicate like this word pay attention to this word like circle it or like aggressively underline a mouse or something like that's how I think I'd use that and i'm like i just wouldn't do that but if i were trying to do even if i were trying to no see because it's not it's different from from the whiteboard feature yeah i don't know I just i think that would only be useful like let's say if you're a biology student and you're trying to talk about different parts of a diagram or something and then it helps to kind of be like see this one right here this is what i'm talking about or something like that but if i'm just mostly trying to convey meaning through words then it doesn't really need that extra"

% \subsection{Tools for Receiving and Giving Feedback}
% 2.4

% 2.4.1
% \noindent {\bf Rating Feedback.} 
% Participants were asked if they would be comfortable and if they would use various forms of feedback rating systems. This covered rating systems that would be only visible to the students who were teaching, or public ratings to everyone in the platform (where the author could be identified or anonymous), and if such systems existed which rating prompts would they include. Some participants mentioned that they may be rated on depth of content (P3, P4, P20), quality of content (P4, P20), clarity of content (P20-21), organization of content (P20), overall presentation (P4), how much help they required (P3), how responsive/adaptive they are (P22), on a numeric scale (P3, P15, P25), on a non-numeric scale from ``low to high" (P23), or ``drop down fields" (P7) that the student can modify (P15).

%removed Jan12: %  comfortable private -----------
% Several participants said they would feel comfortable if the ratings were only visible to the student who was teaching (P2-3, P6-18, P20-25) and one participant said that they would not be comfortable with any form of ratings (P19). P3 said ``it would be a good way to like figure out which improvements I can possibly do and see where I am currently at" and P10 added ``I think that's the only way to improve", ``if I'm participating it's because I want to help other people so I would need that feedback in order to improve." A few participants said that they would be comfortable with this because ``if you're going on the 
% % learning-by-teaching 
% platform, you should be receptive to feedback" (P7), but ``it'd have to be open-ended" (P7), ``allow [students] to make comments" (P6-7) and explanations (P2, P8), ``rather than just having ... drop-down fields" (P7) ``because of a lot of misinterpretation/miscommunication [can be taken] the wrong way" (P7), ``rating could vary quite a bit from one person to the next" (P8), and comments could be ``clearer if this is a short amount of time that you're meeting" (P6). P18 also said that they would use this if it has ``the option for anonymity because [they] think that gives people a different level of confidence ... to speak freely". 
% removed to cut down pages:In addition, P15 said that the platform ``would need to regulate it in some way" and ``maybe you need a verified account". Despite being comfortable with the feature, two participants said that they would not use it (P9, P13) because P13 they ``don't know that it gets at the point of learning-by-teaching because the theory is that you don't actually know it that well and so you have to teach it to know it so theoretically your teaching won't be that good so it might create this sort of weird tension between already knowing everything to have a perfect teaching experience and the people that are kind of like I don't know this but I'm just gonna try to work through it with someone by teaching" they also said that ``if I got rated and I might feel pressured to give a flawless presentation, like do my hair, I don't know". Similarly P13 said that they ``would definitely read it but I feel like it would take away from the learning part and I would just be so focused on like what people think of me which would not be helpful" and P16 said that ``the point is that you're teaching---well or just that you thought about I---through the process of figuring out how to teach someone and it doesn't matter if you're good at it."
% P2 ``R: okay if they were ratings with feedback would you use it if it was private just to you P: yeah yeah because like it's not just about like oh like i don't want people to see like my shitty rating it's just that it's really useless to have like a three star rating but not know why so it's like because i know a lot of places have like oh rate us like out of five and then you can leave optional feedback but most people obviously don't want to leave type words but like that's like pretty useless for like growth and it would just make me feel shitty and like isn't useful so i would only like feel comfortable and use it if it was ratings with mandatory feedback or you just can't leave a rating"
% removed for Aug 22 : new line
% hesitant public --------------------
% removed Jan12: Various participants were hesitant to use and feel comfortable about public ratings in the platform (P2, P3, P6-9, P16, P18, P25) since there would be more ``pressure" (P3), more nervousness (P3, P8), and it would feel ``like a teaching app more than a learning-by-teaching app" (P6). Additionally, there could be more ``bias" ratings (P7, P25), and people ``might troll you and give you like no stars at all" (P25). 
% removed for Aug 22 : P25 explained that listeners might ``ask a question and you don't know but it's not too relevant to what you're talking about" so they would ``take it with a grain of salt".  Another participant said they would then not like to be paired with somebody with a ``two-star rating" as to not listen to ``bad" teaching (P6). One participant, P8, said that 'it would probably keep me from participating more than encourage me to participate even if the ratings were good". Lastly, P14 said that they would be comfortable with it but less and they would use it if there was the option for anonymity.
% removed for Aug 22 : new line
%  comfortable public --------------------- P4-5, P12, P15, P17, P20-23 (but have the option) , P10, 11 13 (but slightly less)
% removed Jan12: Some participants said that they would be comfortable with and would use public rating systems (P4-5, P12, P15, P17, P20-23) and some participants would feel slightly less comfortable but would still use it (P10-11, P13) for making informed peer matching decisions (P4, P5), for transparency (P5) and honesty (P5). 
% removed for Aug 22 : P4 explained that they would be OK with sharing their rating with others so that ``it would make it easier for them to pick me as someone to teach them ... before they choose my session they should be able to see my rating, so I think that's fair." P12 added, ``I feel like, would make it easy for people who already know the subject to learn" on the flip side ``I would worry about people who were trying to teach things that they particularly struggled with and we're trying to like very deeply learn about these subjects in through the like learning-by-teaching and having difficulty getting good ratings" so ``it would take the focus towards here's like a co-teaching platform versus here's a platform to learn by teaching" however ``I'd probably use it because I have enough confidence in my teaching abilities".
% removed to cut down pages:Another participant said that they would feel comfortable with it, but slightly less than private ratings since it ``puts more emphasis on like competition and like just like the toxic part of social media." However, P23 said that ``if it's all over the platform uh is forced and the platform is a very small community for example like 50 to 75 to 100 people I guess giving having public ratings are are okay." Some participants preferred public ratings because they thought that ``it's much easier to gain user trust in a community rating system" (P22) and if they were to be matched with someone ``[they] would want to look at this person rating before attending" (P21).

% removed Jan12: \noindent {\bf Feedback Forms.} 
% yy
% P2-14, 16, 18-19, 21-25
% removed Jan12: Participants were then asked how they would feel about giving and receiving feedback through a form. In terms of what feedback is most useful, P10 would expect to see feedback criteria like ``organization", ``time management", ``friendliness", ``competence in explaining the content", ``how much knowledge [the teachers] have about what they are trying to teach", and a freeform field.
% removed for Aug 22 : However, P10 expects to see ``a box for people to write whatever feedback they want", instead of having any specifically prompted feedback. 
% removed Jan12: P11 said that open-ended feedback would be more thoughtful (as compared to people ``mindlessly circling" options on a form). Another participant, P21 said they would use this in combination with ratings if they could be anonymous.
% removed for Aug 22 : as such they would ``trust the [open-ended] feedback more and take it to be more genuine and sincere." 
% removed Jan12: In general, participants who said they would feel comfortable and would use feedback forms (P2-14, P16, P18-19, P21-25) would also want to see some feedback prompts including: learning/teaching style (P14, P22-23), ability to answer questions (P16), and visual/presentation material (P9, P16) as long as the form is not too time consuming (P24-25). Some also said that they would prefer this method over rating systems (P2, P9, P11, P14) and one explained that they would ``trust" the feedback more (P11). Lastly, P12 would like both the teacher and the listener to take part in filling out the form to help with understanding what they each thought about it or what could be improved, such as how ``engaged" they were.
% removed for Aug 22 : Lastly, P12 said that you would want both participants to learn more (both the one doing the learning-by-teaching and the listener), ``so I guess both parties would have to probably take a post session form about the session and probably about their partner as well" to help with understanding what they each thought about it or what could be improved such as how ``engaged" they were.
%  others with good information which could be quoted: p4, 6, 8, 9, 12, 16(optional)
% not yet included whether participants wanted pre-selected prompts or to create their own
% removed to cut down pages:Two participants said that they would prefer a rating system over a feedback form (P15, P20). P20 said that they would feel comfortable with using this but would probably send out a rating instead unless they wanted to include more details and P15 said they would like to be able to add comments to the rating system if needed. P20 also explained that this would save time. However, P17 said that they would feel comfortable with feedback forms but would not use it.

% removed Jan12: \noindent {\bf Feedback Saved in History Tools.} 
% Participants were also asked about a history tool designed to view and access previously taught session recordings, and to save student's questions.
% % session req
% Several participants said they would feel comfortable having their sessions saved and would use the tool (P2-8, P12, P14, P16-20, P22-24) to be able to view previously taught content, check for areas of improvement (P3, P6), re-watch clips of well explained segments (P4), and to enable asynchronous input from the listener (P5, P19), check if you would be ``interested" in pairing with that peer based on past recordings (P14), and to follow up with comments (P19). Participants P2, P3, and P8 also said they would be OK with sharing this with the students and P12 agreed given that there is ``consent to be recorded for both parties". Other conditions included having the choice to make it public or not (P2, P7, P16-15, P22), have the ability to ``take it down" (P8) or ``delete" it (P22) when they want to. P7 explained that they would not want others ``to be able to like hang on to a copy of me explaining something or struggling to explain something for like forever”. 
% removed for Aug 22 : For example, P7 said they would want it up for ``maybe like a day or two because ... it would be good to like have the flexibility to keep it on there forever", however, ``I would not necessarily like for them to be able to like hang on to a copy of me explaining something or struggling to explain something for like forever so maybe not”. 
% removed for Aug 22 : Another participant talked about the benefits of having sessions publicly shared, P14 said ``it's almost like a verification that this person is like a valid teacher. I don't know why but I would trust someone with more recorded sessions than none because it kind of shows they've been doing it longer and then also like if you were interested in how they teach then you could go back and see other teachings so you could use them as a source of information rather than just like a one-stop shop."
% Session req
% Yy % P17 P18 P20 P23 P24
% P2 - ok if it’s shared with student
% P3 check points you can improve on - share with students
% P4 - explained well and you wanna recap
% P5 - good for stu not teacher and for asynch
% P6 - if they looked at feedback and then wanted to reference the session forget 
% P12 - given there is consent from both parties 
% P19 yes for both parties to go back and comment
% P16 as long as they had the choice to make ti public or not
% P22 yes if able to delete it when wanted and could control who sees it
% P7 -(would not want it shared for more than a day or two with the ppl in the session “i would not necessarily like for them to be able to like hang on to a copy of me explaining something or struggling to explain something for like forever so maybe not”
% P8 (ok with shared if ability to take down)
% P14 both as stu and teacher more trust in recordings
% 
% removed to cut down pages:Two participants said that they would be comfortable with this feature but would not use it (P10, P13) due to it being too time consuming (P10, P13) or because when they teach they generally remember what was said (P13, P25). P10 explained that it would be a lot of work to go through and re-watch, especially if the sessions are ``decently long", by which he means 20 minutes. P11 said that they would be fine with this tool, however, they wouldn't watch videos of themselves as it would be ``very cringy"; instead of struggling through something, they would prefer to ``just do another session instead and continue to further [his] learning that way". Likewise, they would not be comfortable for other people to be able to re-watch his previous teaching. They said, ``if I was paired with somebody [where] we were trying to learn the same thing, and then they had a really good explanation of something, I'd go watch their video again just to solidify things; but ... I don't want myself recorded." One participant, P21 said that they would not be comfortable with this but they would look at it for learning purposes. Lastly, P25 said that they would not use it and would not be comfortable with this feature.
% P9 no awkward - audio might be better less self-conscious
% P10 comfortable but no too time consuming
% P11 fine with it but wouldn’t watch it cause cringe
% P13 comfortable but would not use generally you remember what you teach too time consuming even on x2 speed
% P21 uncomfortable but would look at it
% P25 no not comfortable

% ---------------------------------------------------------save qs
%removed Jan12:  Another feature that was included in this history tool was a method for saving answered or unanswered questions in the 
% % learning-by-teaching 
% LbT sessions. Various participants said they would use this and would be comfortable with it (P2-4, P6-9, P11-23) so that they could ``brush up" on areas of improvement (P2, P11), follow up with the feedback (P2, P4), and to see other peers' answers to questions (P13). P11 explained that they would find saved student questions useful because ``it gives me a point of reference to refer back [to see] where the gaps in my knowledge were and [allow him to work on] a second attempt [to] close those gaps." However, P2 noted that they would not be sure if other listeners who shared questions would be comfortable having it saved, and P15 would like to have consent from all parties. Other conditions included being able to make your questions anonymous or not (P16, P19), having visibility control to specific users (P22), and being able to delete questions (P22).
% removed for Aug 22 : new line
% removed for Aug 22 : One participant (P9) said that they would prefer to have the questions saved over the whole sessions so that they would save time instead of having to scrub through a video. 
% removed Jan12: P9 and P8 said it would be helpful and save time to quickly find specific questions, and P8 explained that ``it's basically like taking notes for you" and it ``keeps a log of what really stood out to the participants or what they didn't understand". Similarly, P10 thought this, and would use it if there was a way to timestamp questions by showing a symbol along a timeline.
% removed for Aug 22 :Similarly, P8 said ``I think that would be really helpful. It's basically like taking notes for you---at that point---which is great because it keeps a log of what really stood out to the participants or what they didn't understand, which would be helpful to have notes on.” They would also want to be able to ”mark off the ones that [they've] already addressed or the ones that are irrelevant.” 
% removed Jan12: Two participants thought it would be better to turn this into an FAQ section (P4, P15) where various peers can share answers and follow up with each other. A few participants said they were comfortable with having their questions saved, but they may or may not refer to them (P10, P24-25) and one explained that they prefer addressing it in the moment (P24). One participant (P5) said that they would not use it due to it being a ``waste of time". 
% removed for Aug 22 :P10 had the idea that they would use if if there was a way to timestamp questions. They said ``I'm thinking like if you click on like a lesson video from the past and then you know like where there'd be a scroll bar to kind of scroll through the video and maybe there's like some sort of symbol like along the timeline that kind of marks like a question or maybe like a different topic that you were like teaching during the lesson, if that makes sense."
% 
% Many participants said that they would be comfortable using receiving some sort of rating on their teaching (P10, P11), especially if the rating is kept private. Both P10 and P11 said that they would be less comfortable with the lesson rating being public, but that would not deter them from wanting or using it. Many participants see the benefit of verbal feedback; they recognize that feedback can ``improve [their own] teaching abilities and make sure [they are] helping people to the best of [their] ability" (P10). Participants (P10) are also comfortable with live feedback prompts, prompts that are determined by the teacher and sent out to learners listening to the session.

% 2.4.4
% removed Jan12: \noindent {\bf Post-session Annotated Feedback.} 
% Lastly, we asked participants how they would feel about using a specific tool for post-session annotated feedback. In the history tool---where users can see your saved sessions---users would be able to select a session, then click on a timestamp of that recording, then a dialogue box would appear and the user could write feedback and/or select a category describing the type of feedback they wanted to give (e.g., correct content, incorrect content, area of improvement, etc.). Once saved, the timeline would display symbols over those timestamps to be able to reveal the feedback when selected and jump to that spot.
% % removed for Aug 22 : new line
% Of the 23 participants who were asked, most of them said they would be comfortable with such a tool and would use it (P3, P5-11, P13, P15-23), a few others said they might use it (P4, P12, P14, P25), and one said that while they would be comfortable with it, they would not use it (P24). P20 said that they would use it to comment on areas where content could be expanded, to indicate which sections are more important for a course, where an explanation could be slower, or where an image could have been used, and P22 would use it to identify knowledge gaps. One participant, P3, thought that this would be useful for the listener and also for the one doing the teaching.
% % removed for Aug 22 :, saying ``if I accidentally misspoke or something was wrong yeah then going back and fixing it would be useful". 
% P11 can see the benefit of an annotation tool where you can provide feedback to others: ``if a person seemed frustrated, I would [tell them], 'You're doing so good! Don't worry, you got this!'", ``as a way to encourage people", and to provide ``critiques".
% removed for Aug 22 : or if they were really excited or showing enthusiasm about something, ``I'd use it as a way to encourage people. And then, I'd also use it as a critique---if somebody ... weren't certain of what they were saying, and [if] I actually had the knowledge, then I could share that with them." 
% Yy 3 5-11, 13, 15-23
% removed for Aug 22 : new line
% removed to cut down pages:P7 said that they used something similar for a course where they had oral presentations where the professor gave feedback associated to a timestamp finding this to be very helpful. Another participant (P8) said that it would be helpful specifically for math and chemistry courses ``when you're just trying to teach and you're writing out all of these formulas and then someone says you missed the exponent here and you're not going to know where that is unless they can point it out so having that feature would be really helpful." Similarly, P18 said that they would use if for ``very specific feedback... I think that'd be probably one of the more effective tools because then you can address exactly where and you're going right and wrong." P16 said that this would be useful for submitting ``those markers live" for an opportunity to learn or clear up misunderstandings the listener may have had when providing feedback.
% removed for Aug 22 : new line
% removed Jan12: A few participants said that they would use it upon certain conditions. P10 said they would use just the textbox without selecting specific prompts or feedback types. 
% % removed for Aug 22 :Another participant said that they would use it, however, they ``don't know how well other people would use it" (P13). 
% P23 said that it could be ``demotivating" if there is no ``constructive feedback" and the annotation only indicates if a timestamp was good or bad. Another participant (P15) said that they would like to use this too if there are only a few people in the session, ``like five people or less" otherwise it could ``cause some confusion".
% removed for Aug 22 : Lastly, P21 said they would use this but that it is ``actually a pretty new tool" and they tend to be a ``late technology adopter" so they would wait for other people to try it first. 
% removed for Aug 22 : new line
% M 4 12 14 25
% removed Jan12: The participants who said they might use it, said this due to not always seeing ``the value in pairing a comment with a timestamp" (P12), preferring to make their own notes separately (P14), or due to time constraints (P25).
% removed for Aug 22 : since they don't see themselves re-watching videos too often or going in depth and annotating (P25).
% removed to cut down pages:Similarly, P24, said they would not use this tool because they are ``gonna go on this website to ...teach someone something, to confirm to myself whether I know it or not, and I don't think beyond ...the teaching session that I would like spend much time on the website doing things like annotating and going over stuff ... I would use it for the ability for it to connect me with people who want to listen to me ... to teach, get feedback, and move on." Lastly, P4 said that they would rather just build new content if they were the one doing the learning by teaching since it could be a ``bit messy" but they would use it if they were the listener giving feedback.
% Yn 24


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Learning by Teaching Community %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  moved to previous section
















% from thesis and removed
% \section{A LbT Platform Prototype}
% % validating (but not really) design implications
% % LbT Through collaborative Deconstruction
% % https://www.overleaf.com/project/602716b0eeecb422fdb4819f

% To begin understanding how to design a LbT Platform for university students we built a prototype that begins to incorporate design solutions presented in Chapter 5 and ran a pilot study with 12 students enrolled in the Winter 2021 graduate offering of \emph{CS889: Masterclass in Human-Computer Interaction: Educational Technology} at the University of Waterloo.

% \noindent{\bf Prototype System Design. }
% \begin{figure}[h!]
% \centering
%   \includegraphics[width=1\columnwidth]{ListCreation.PNG}
%   \caption{MicroLbT}~\label{fig:listCreation}
%   \label{prototype}
% \end{figure}
% We present \emph{MicroLbT} (Figure \ref{prototype}), a prototype platform that supposed collaborative LbT in an online context. This platform incorporates micro learning (discussed in Chapter 5) where a group of peers simultaneously take the role of the teacher and learner in LbT to answer a shared question by collaboratively deconstructing and sequencing segments of an explanation and then recording instructional and time-limited audio for each segment. More specifically, the platform scaffolding provides the students with an audio segment creation and organization tool where each segment in a sequence holds both the micro-teaching segment name and its corresponding explanation recordings. MicroLbT segments can be easily added, rearranged, and modified to restructure the explanation as many times as group members require. Users can also rearrange the order of segments by simply clicking and dragging a segment. This reordering is preserved so that other group members can work on the updated sequence. The ability to restructure segment orderings supports learner-teachers as they make clarifying edits to the explanation, much like in the multi-component model of micro learning \cite{swertz2006customized}.

% Previous work further specifies how having screen-capturing and voice recording instead of videotaping reduces the Hawthorne effect and that subjects may be more shy in front of a video camera than a microphone, since the latter is less conspicuous \cite{xu2005dialogbasedprotocol}. Since audio recordings could ensure a greater degree of comfort, we chose to enable students to share teaching segments via audio recordings. 

% The goal of this platform is to support the LbT Crash and Learn process to become comfortable with making mistakes and learning from them. Therefore, we have designed it so that students can listen to the clips of other group members in order to learn from them and iteratively improve their own explanations. A participant can both listen to and record their own clips for a segment. To reduce nervousness and perfectionism in recordings, we allow students to overwrite their own clips and edit the clip's label at any time, which is a technique that has been shown to reduce anxiety in language tutors in previous work \cite{poza2011effects}. 

% \noindent{\bf Pilot Study. } To understand the effects of recording time-restricted LbT audio segments to encourage micro learning, we conducted a within-subject pilot study conditioned on the segment length. One experimental condition enabled the students to create thirty-second learning-by-teaching segments, while the other condition allowed the students to create one-minute learning-by-teaching segments. We were interested in evaluating whether participants will feel a reduction of nervousness around teaching material incorrectly when the segments limit the length of time for which a student could potentially be incorrect, compared to the condition where they must record longer segments and could potentially be incorrect for longer lengths of time. Participants confidence levels were recorded in the platform after each recording as well as in a post-pilot-study survey. 

% The preliminary results suggested that deconstructing a topic into smaller subtopics could increase confidence in students and that interactions with content from group members could have positive impacts on confidence. Furthermore, it was also observed that given a fixed duration to interact with the system, shorter time limits free participants to explore peer's responses on the platform more. Future directions of this pilot study could focus on improving the prototype interface to enable the grouping of shorter audio segments into larger units, supporting the learning of various domains, and executing a more thorough experimental study to get enriched and reliable results. From the pilot study results, this platform shows promise for facilitating online collaborative LbT beginning with incorporating micro learning methods.


% % a few paragraphs explaining prototype and pilot study

% % from the conclusion: to be updated
% % This work presented MicroLbT, a collaborative online LbT platform that facilitates learning and teaching through time-limited audio segments. In a pilot study with 12 participants organized into four groups of three, participants were asked to collaboratively deconstruct an explanation prompt into various segments, by providing explanations for each segment within 30-seconds or 60-seconds which formed the two conditions of the study. We investigated the differences in self-reported confidence between the two conditions. We also explored how LbT in a group setting can affect confidence levels in regards to correctness. The preliminary results show that deconstructing a topic into smaller subtopics can increase confidence in learner-teachers and that interactions with content from group members can have positive impacts on confidence. Furthermore, it was also shown that given a fixed duration to interact with the system, shorter time limits free participants to explore the platform more. Future directions of this study could focus on improving the interface to enable the grouping of shorter segments into larger units, supporting the learning of various domains, and having a longer study duration to get more enriched results. From the pilot study results, this platform shows promise for facilitating online collaborative LbT.






 
